SPION: Layer-Wise Sparse Training of Transformer via Convolutional Flood Filling

Sparsifying the Transformer has garnered considerable interest, as training the Transformer is very computationally demanding. Prior efforts to sparsify the Transformer have either used a fixed pattern or data-driven approach to reduce the number of operations involving the computation of multi-head attention, which is the main bottleneck of the Transformer. However, existing methods suffer from inevitable problems, such as the potential loss of essential sequence features due to the uniform fixed pattern applied across all layers, and an increase in the model size resulting from the use of additional parameters to learn sparsity patterns in attention operations. In this paper, we propose a novel sparsification scheme for the Transformer that integrates convolution filters and the flood filling method to efficiently capture the layer-wise sparse pattern in attention operations. Our sparsification approach reduces the computational complexity and memory footprint of the Transformer during training. Efficient implementations of the layer-wise sparsified attention algorithm on GPUs are developed, demonstrating a new SPION that achieves up to 3.08X speedup over existing state-of-the-art sparse Transformer models, with better evaluation quality.

==> algorithms/sparseattentionfor.tex <==
\begin{algorithm}[!ht]
\caption{GPU implementation of sparse MHA for forward propagation on host \gm{remove this algorithm later on}}
\label{alg:spattnfor}
\footnotesize
\KwIn{$Q, K , V, P, scale$ }

$S^r \gets \text{cusparseSDDMM}(Q,K,P.row\_ptr,P.col\_idx,P.values)$

$S^s \gets \text{SparseSoftmax}(S^r, P.row\_ptr, P.values, scale)$

$S^c \gets \text{cusparseSpMM}(S^s,V,P.row\_ptr,P.col\_idx,P.values)$

\end{algorithm}

==> algorithms/sparseattnback.tex <==
\begin{algorithm}[!ht]
\caption{GPU implementation of sparse MHA for backward propagation on host}
\label{alg:spattnback}
\footnotesize
\KwIn{$Q, K , V, S^s, \nabla S^c,P, scale$ }

\KwOut{$\nabla Q, \nabla K, \nabla V$ }

$\nabla S^s \gets \text{cusparseSDDMM}(\nabla S^c, V, P.row\_ptr, P.col\_idx, P.values)$

$\nabla S^r \gets \text{SparseSoftmaxBack}(\nabla S^s, S^s, P.row\_ptr, P.values, scale)$

$\nabla Q \gets \text{cusparseSpMM}(\nabla S^r, K, P.row\_ptr, P.col\_idx, P.values)$

$\nabla K \gets \text{cusparseSpMM}(\nabla S^r,Q, P.row\_ptr, P.col\_idx, P.values)$

$\nabla V \gets \text{cusparseSpMM}(\nabla S^r,\nabla S^c, P.row\_ptr, P.col\_idx, P.values)$

\end{algorithm}

==> algorithms/sparsesoftmaxback.tex <==
% \begin{algorithm}[!ht]
% \caption{\textit{BackSparseSoftmax}() kernel on GPUs}
% \label{alg:spsoftmaxback}
% \KwIn{$\nabla S^s, S^s, offsets,cnt\_mat, nnz, scale$}

% $b\_cnt \gets cnt\_mat[threadIdx.x]$

% $b\_idx \gets blockIdx.x \times nnz + offsets[threadIdx.x]$

% $\nabla sum \gets 0$

% \For{$k = 0$ to $b\_cnt-1$}{
% $\nabla S^s[b\_idx + k] \gets \nabla S^s[b\_idx + k] \times S^s[b\_idx + k]$

% $\nabla sum += \nabla S^s[b\_idx + k]$
% }

% \For{$k = 0$ to $b\_cnt-1$}{
%     $\nabla S^r[b\_idx + k] \gets (\nabla S^s[b\_idx + k] ]\times (S^s[b\_idx + k] \times \nabla sum)) \times scale$
% }

% \end{algorithm}

\begin{algorithm}[!ht]
\caption{SparseSoftmaxBack() kernel for backward propagation on GPUs}
\label{alg:spsoftmaxback}
\footnotesize
\KwIn{$\nabla S^s, S^s, P, scale$}


$warp\_id \gets \lfloor threadIdx.x / warp\_size \rfloor$

$lane \gets threadIdx.x  \%  warp\_size$

%$b\_cnt \gets cnt\_mat[warp\_id \% L]$

$b\_cnt \gets P.row\_ptr[(warp\_id + 1) \% L] - P.row\_ptr[warp\_id \% L]$

$b\_idx \gets \lfloor warp\_id/L \rfloor \times P.values + P.row\_ptr[warp\_id \% L]$

$\nabla sum \gets 0$

\For{$k \gets lane$ \KwTo $b\_cnt-1$ \KwBy $warp\_size$}{
$\nabla S^s[b\_idx + k] \gets \nabla S^s[b\_idx + k] \times S^s[b\_idx + k]$

$\nabla sum \gets sum + \nabla S^s[b\_idx + k]$
}

$\nabla sum  \gets warp\_reduce\_sum(\nabla sum)$

\For{$k$ = $lane$ \KwTo $b\_cnt$-1 \KwBy $warp\_size$}{
    $\nabla S^r[b\_idx + k] \gets (\nabla S^s[b\_idx + k] ]\times (S^s[b\_idx + k] \times \nabla sum)) \times scale$
}

\end{algorithm}

==> sections/acknowledgements.tex <==
\section*{Acknowledgments}

The preferred spelling of the word ``acknowledgments'' in America is without 
an ``e'' after the ``g''. Avoid the stilted expression ``one of us (R. B. 
G.) thanks $\ldots$''. Instead, try ``R. B. G. thanks$\ldots$''. Put sponsor 
acknowledgments in the unnumbered footnote on the first page.


==> tables/attntime.tex <==
\begin{table}[]
\begin{tabular}{|c|cc|cc|}
\hline
                                                       & \multicolumn{2}{c|}{lra-image}       & \multicolumn{2}{c|}{lra-text}        \\ \hline
                                                       & \multicolumn{1}{c|}{Original} & Ours & \multicolumn{1}{c|}{Original} & Ours \\ \hline
\begin{tabular}[c]{@{}c@{}}GEMM\\ (SDDMM)\end{tabular} & \multicolumn{1}{c|}{}         &      & \multicolumn{1}{c|}{}         &      \\ \hline
Softmax                                                & \multicolumn{1}{c|}{}         &      & \multicolumn{1}{c|}{}         &      \\ \hline
\begin{tabular}[c]{@{}c@{}}GEMM\\ (SpMM)\end{tabular}  & \multicolumn{1}{c|}{}         &      & \multicolumn{1}{c|}{}         &      \\ \hline
\end{tabular}
\caption{Attention Mechanism Operations Execution Time Comparison}
\label{tab:attntime}
\end{table}

==> tables/finetuning.tex <==
\begin{table}[]
\centering
\begin{tabular}{|c|c|c|}
\hline
Model          & CIFAR-10 & FGVCAircraft \\ \hline
\proposed{}-CF/15 & 95.563  & 59.315       \\ \hline
\proposed{}-CF/25 & 95.934  & 59.766       \\ \hline
\proposed{}-CF/35 & 96.424  & 60.487       \\ \hline
\end{tabular}
\caption{Comparison accuracy (\%) of fine-tuning ViT model on CIFAR-10 and FGVCAircraft dataset. $\alpha$ in \proposed{}-CF/$\alpha$ indicates the threshold value used in flood filling method.  }
\label{tab:finetuning}
\end{table}

==> tables/inftime.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{|l|l|l|l|l|}
\hline
           & Image & ListOps & Text  & Retrieval \\ \hline
Original   & 23.27 & 40.32   & 37.88 & 73.04     \\ \hline
BigBird    & 37.96 & 47.56   & 32.95 & 59.23     \\ \hline
Reformer   & 23.79 & 24.91   & 19.67 & 28.33     \\ \hline
Ours(conv) & 21.03 & 21.04   & 17.81 & 27.59     \\ \hline
Ours(ff)   & 21.33 & 24.03   & 17.25 & 26.80     \\ \hline
Ours       & 21.46 & 23.14   & 17.56 & 27.02     \\ \hline
\end{tabular}
\caption{Execution Time(ms) of Single Inference Step}
\label{tab:inftable}
\end{table}

==> tables/mhatime.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{|l|l|l|l|l|}
\hline
           & Image & ListOps & Text  & Retrieval \\ \hline
Original   & 11.38 & 23.06   & 23.41 & 37.20     \\ \hline
BigBird    & 27.55 & 23.88   & 14.31 & 21.18     \\ \hline
Reformer   & 8.76  & 9.02    & 5.67  & 8.38      \\ \hline
Ours(conv) & 4.03  & 5.13    & 4.76  & 7.18      \\ \hline
Ours(ff)   & 4.42  & 6.52    & 4.56  & 6.87      \\ \hline
Ours       & 4.34  & 6.56    & 4.59  & 6.91      \\ \hline
\end{tabular}
\caption{Execution Time(ms) of Multi-Head Attention Operation}
\label{tab:MHAtime}
\end{table}

==> tables/sparsitytable.tex <==
\begin{table}[]
\centering
\begin{tabular}{|l|l|l|l|}
\hline
Density & Accuracy & \begin{tabular}[c]{@{}c@{}}Time\\ (ms)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Memory\\ (GB)\end{tabular} \\ \hline
1\%     & 38.333   & 41.298                                              & 2.803                                                 \\ \hline
4\%     & 38.889   & 54.787                                              & 3.177                                                 \\ \hline
10\%    & 39.063   & 83.712                                              & 3.951                                                 \\ \hline
20\%    & 39.583   & 128.589                                             & 5.223                                                 \\ \hline
30\%    & 39.792   & 178.452                                             & 6.510                                                 \\ \hline
40\%    & 40.521   & 228.018                                             & 7.781                                                 \\ \hline
\end{tabular}
\caption{Comparison of classification accuracy(\%), single step training time (ms), and single training step memory consumption (GB) between density on ListOps task}
\label{tab:sparsitytable}
\end{table}

==> tables/trainbreakdown.tex <==
\begin{table}[h]
\centering
\caption{Breakdown of total elapsed time (s) for training \proposed{} on image classification task}
\scalebox{0.9}{
\begin{tabular}{|c|c|}
\hline
              & Elapsed Time (s) \\ \hline
Dense-attention training          & 210.84   \\ \hline
Sparsity pattern generation & 0.65     \\ \hline
Sparse-attention training       & 1673.47  \\ \hline
Total training time              & 1389.31  \\ \hline
\end{tabular}}
\label{tab:trainbreakdown}
\end{table}
